Pilot evaluation of Collection API with PID Kernel Information

As digital data become increasingly available for research, there is a growing awareness of the value of domain agnostic Persistent Identifiers (PIDs) for data. A PID is a globally unique reference to a digital object, which in our case is data. In an ecosystem of connected digital objects, a PID will reference a digital object, and the digital object will be a simple entity, a collection of homogeneous objects, or a set of heterogeneous objects. In this paper, we study two recent recommendations from the Research Data Alliance (RDA) that both address pieces of an ecosystem of connected digital objects. The recommendations address Persistent ID records and representations of collections of data. We evaluate different approaches in where to locate key information about a data collection between these two component solutions.

==> 1_intro.tex <==




==> 2_relativework.tex <==
The academic and industry already develop similar Persistent Identifiers with different semantic and syntax. Paskin \cite{paskin2010digital} pointed out the high level understanding about the DO of the scope, the syntax and the resolution. In his research, he raised up a definition for metadata, DOI Kernel, the minimum set of metadata information specified by the IDF registered with DOI. The DOI Kernel is similar to the PID Kernel Information that we described in this research, excepting that PID Kernel Information contains the \textbf{Backbone Provenance} to enhance the connections to other objects for drawing the Provenance Network. DOI tends to provides abundant information for users to understand the objects.

Archival Resource Key (ARK) \cite{kunze2003towards} presented by Kunze is another approach to make the permanence of object. The ARK is not like other conventional schema (URL, PURL, and URN), it provides three things: object, metadata and provider's commitment. While adding '$?$' to the end of one ARK link, the server would return the human-readable information, for example, the Electronic Resource Citation using Dublin Core Kernel metadata, including who, when, where and what. All these kernel information would help users just understand the object, but not the relationships to other objects. 

The PID Kernel Information of Handle in this research inherits the benefit of Persistent Identifier and try to add more efforts to the data ecosystem, not only referencing to the single object, but also presenting the entire graph of connected objects.

Some other researchers raise the idea about network of provenance, the visualization of connected objects. Zhou \cite{Zhou:2010:EQM:1807167.1807234} discussed their work, ExSPAN, a framework that achieves the network provenance at Internet-Scale. The ExSPAN stores the provenance in a relational table, and try to make a granular relationship graph of objects for efficient query and maintain. The idea of keeping network provenance is quite similar to the research of this paper, but ExSPAN is working on the local use and analysis. However, the research in this paper is forcing on the global scope that building the provenance network for objects, offering efficient approach on publishing and maintaining public objects.

Chen \cite{chen2012visualization} provides a approach to visualize the graph of network provenance captured from streaming data. The research is fully maximizing the benefit of provenance, and use visualization techniques to interact with data object. The idea of representing the network data by using provenance from Chen's research is a good reference to start our research, however, our research wants to make the the Internet Scale of presenting and sharing data, using the minimal metadata information, keeping fine-grain provenance relationship, by using Persistent Identifiers. All these requirements are challenges for current Network Provenance or Provenance Network representation work, and this is the motivation that we do the pilot evaluation on Handle System and Collection API Service, attempting to contribute to the Publishing Ecosystem.

A visualization system, Komadu \cite{suriarachchi2015komadu}, is a tool embedded in other softwares to ingest and present the provenance information while doing workflow. The system is powerful on providing high level understanding of provenance among different object. However, the centralized database and local sharing mechanism restricted the data sharing on Internet.
